Understanding the Role of Adaptivity in Machine Teaching: The Case of Version Space Learners

In real-world applications of education, an effective teacher adaptively chooses the next example to teach based on the learner's current state. However, most existing work in algorithmic machine teaching focuses on the batch setting, where adaptivity plays no role. In this paper, we study the case of teaching consistent, version space learners in an interactive setting. At any time step, the teacher provides an example, the learner performs an update, and the teacher observes the learner's new state. We highlight that adaptivity does not speed up the teaching process when considering existing models of version space learners, such as "worst-case" (the learner picks the next hypothesis randomly from the version space) and "preference-based" (the learner picks hypothesis according to some global preference). Inspired by human teaching, we propose a new model where the learner picks hypotheses according to some local preference defined by the current hypothesis. We show that our model exhibits several desirable properties, e.g., adaptivity plays a key role, and the learner's transitions over hypotheses are smooth/interpretable. We develop efficient teaching algorithms and demonstrate our results via simulation and user studies.

==> random_notes.tex <==
\newpage
\section{Teaching Algorithm for $k$-disjoint objects}
\yuxin{More accurately, we are teaching a hypothesis class which has $k$ different types of hypotheses, with shortcuts between different types. We need a better phrase for this hypothesis class -- probably not ``$k$-disjoint objects''.}


Main idea:
\begin{itemize}
\item if $\hstar$ is in a class of higher complexity than $\hypothesis_0$, then we first teach the shortcut in the class of $\hypothesis_0$, add a rule to move to the next class; iterate over such process until reaching the class of $\hstar$. Then we teach $\hstar$ from a hypothesis in the same class.
\item if $\hstar$ is in a class of lower complexity than $\hypothesis_0$, then we first teach the shortcut in the class of $\hypothesis_0$, remove an object to move to the next lower-complexity class; iterate over such process until reaching the class of $\hstar$. Then we teach $\hstar$ from a hypothesis in the same class.
\end{itemize}
Let $\shortcut(\hypothesis\given \hstar)$ denote the set of ``shortcut'' hypotheses from $\hypothesis$ to $\hstar$. The shortcut set $\shortcut(\hypothesis \given \hstar)$ provides a set of candidate hypothesis on the optimal path from $\hypothesis$ to $\hstar$. We assume that the shortcut function $\shortcut(\cdot \given \hstar)$ is given to the teacher by a domain expert. For example, for teaching 2 disjoint rectangles, we have


previous version:
\begin{align}
  s(\hypothesis \given \hstar)=
  \begin{cases}
    \hypothesis^* &\text{~if~} \cls(\hypothesis) = \cls(\hypothesis^*)
    \\
    h'\in \{\tilde{h}: \tilde{h}\in M_1, \tilde{h} \text{~shares 1 rectangle with~} h^*\} &\text{~if~} \hypothesis\in M_1, \hypothesis^*\in M_2
    \\
    h'\in \{\tilde{h}: \tilde{h}\in M_2, \tilde{h} \text{~shares 1 rectangle with~} h^*\} &\text{~if~} \hypothesis\in M_2, \hypothesis^*\in M_1\\
  \end{cases}
\end{align}

current version:
\begin{align}\label{eq:shortcut-2-rectangle}
  \shortcut(\hypothesis \given \hstar)=
  \begin{cases}
    \{\hstar\} &\text{~if~} \cls(\hypothesis) = \cls(\hstar)
    \\
    \{\hypothesis': \cls(\hypothesis') = \cls(\hypothesis) \wedge \hypothesis' \text{~shares 1 rectangle with~} \hstar\} &\text{~if~} \cls(\hypothesis) \neq \cls(\hstar)
  \end{cases}
\end{align}
Here, $\cls: \hypotheses \rightarrow \{M_1, M_2\}$ denotes the class membership function of a hypothesis.

Fix a hypothesis $\hypothesis$ and version space $\Hypotheses$, we define the rank function $\rank(\cdot \given \hypothesis, \Hypotheses): \Hypotheses \rightarrow \nats$ as the number of hypotheses in $\Hypotheses$ that are more or equally preferred to $\hypothesis'$, assuming that the learner is at $\hypothesis$:
\begin{align}
  \rank(\hypothesis'\given \hypothesis, \Hypotheses) = |\{{\hypothesis''}: \sigma(\hypothesis'', \hypothesis) \leq \sigma(\hypothesis', \hypothesis) \} \cap \Hypotheses|
\end{align}
Consider the following objective:
\begin{align}
  f(\example \given \hypothesis, \Hypotheses) = \min_{\hypothesis'\in\shortcut(\hypothesis\given \hstar)} \rank(\hypothesis' \given \hypothesis, \Hypotheses(\{\example\}))
\end{align}
which returns the rank of the closest ``shortcut'' hypothesis, after the learner receives example $\example$ at hypothesis $\hypothesis$ and version space $\Hypotheses$.

\begin{algorithm}
  \caption{The adaptive teaching algorithm for k-disjoint objects}\label{alg:k-objects}
  \begin{algorithmic}
    \STATE {\bf Input:}
    Target hypothesis $\hstar$,
    version space $\Hypotheses$,
    shortcut sets $\shortcut(\hstar \given \hypothesis)$ from any $\hypothesis\in \Hypotheses$ to $\hstar$,
    preferences $\sigma(\cdot, \cdot)$,\\
    (optional) initial hypothesis $\hypothesis^0$.
    \STATE Initialize $t \leftarrow 0$, $Z \leftarrow \emptyset$, $\Hypotheses^0 \leftarrow \Hypotheses$
    \WHILE{$\rank(\hstar\given \hypothesis^t, \Hypotheses^t) \neq 1)$}
    \STATE Observe $h^t$
    \STATE $\example^{t+1} \leftarrow \argmin_\example f(\example \given \hypothesis^t, \Hypotheses^t)$ \\\COMMENT{\commentfmt{$\drsh$ greedily pick the next teaching example that brings learner to the closest ``shortcut'' hypothesis}}
    \STATE $\Hypotheses^{t+1} \leftarrow \Hypotheses^t\cap \Hypotheses(\{\example^{t+1}\})$
    \STATE (Learner makes a move according to $\sigma(\cdot, \cdot)$ and $\Hypotheses^{t+1}$.)
    \STATE $Z\leftarrow Z \cup \{\example^{t+1}\}$
    \STATE $t \leftarrow t+1$
    \ENDWHILE
    \STATE {\bf Output:} Sequence of teaching examples $Z$
  \end{algorithmic}
\end{algorithm}

A few remarks are in order:
\begin{itemize}\denselist
\item At any time step $t$, the teacher (\algref{alg:k-objects}) tries to steer the learner to the closest shortcut of $\hstar$.
\item Having access to the shortcut function $\shortcut(\cdot\given \hstar)$, to some extend, allows the teacher to do non-myopic planning.
\item If $\forall \hypothesis \in \Hypotheses, \shortcut(\hypothesis \given \hstar) = \{\hstar\}$, i.e., the shortcut set being the target hypothesis itself, then \algref{alg:k-objects} reduces to the rank greedy algorithm, which further reduces to greedy-SetCover (resp. greedy-PB-SetCover) with the uniform preference function $\sigma^u$ (resp. global prefenece function).
\item Adaptivity is important for \algref{alg:k-objects}; without observing $\hypothesis^t$, the shortcut set could grow very big.
\end{itemize}

\yuxin{The above algorithm works for teaching 2-disjoint rectangles if we plug in the shortcut function $\shortcut(\cdot \given \hstar)$ defined in Eq.~\eqref{eq:shortcut-2-rectangle}. Still need to workout the exact number of teaching examples required, but I'm optimistic that it gives us the same number as the non-myopic rectangle-specific algorithm.}

\begin{align*}
  \cost^\opt(\hypothesis, \hypotheses, \example)
  &= 1 + \max_{\hypothesis'\in f(\hypothesis,\hypotheses,\sigma, \example)}\heuristics^\opt(\hypothesis', \hypotheses\cap \Hypotheses(\example)),\notag \\
  &= 1 + \max_{\hypothesis'\in }, \notag \\
  &\text{where~} \heuristics^\opt(\hypothesis, \hypotheses) = \min_{\example}\cost^\opt(\hypothesis, \hypotheses, \example)
\end{align*}


\subsection{A Concrete Example: Teaching 2-disjoint rectangles}
% We use the following preference function which is defined through the number of edge movements.
% \begin{align*}
%   \sigma(\hypothesis', \hypothesis) =
% \end{align*}

% For the 2-rectangle class, the $\rank$ function is specified through the following rules:
% \begin{itemize}
% \item Hypotheses with the same number of rectangles are ranked in lexicological order of $\{\text{Edgediff}(\hypothesis, \hypothesis'), \text{SymmetricDiff}(\hypothesis, \hypothesis')\}$. Here, $\text{EdgeDiff}(\hypothesis, \hypothesis')$ is defined as the minimal number of edge movements required to transfrom $\hypothesis$ to $\hypothesis'$:

% \item
% \end{itemize}

\paragraph{Implementation Notes}
\begin{itemize}
\item Consider the discretized space, for example $(0,0)$ to $(100,100)$,  A hypothesis (2 disjoint rectangles) is represented by the coordinates of the four corners, i.e., lower left and upper right corners of the two rectangles: $(x_{11}, y_{11}, x_{12}, y_{12}, x_{21}, y_{21}, x_{22}, y_{22})$.
\item \yuxin{TODO: how to enumerate the version space? is it necessary to enumerate?--- Total number of hypothesis is up to order $\bigO(100^8)$ (we still need to rule out the hypotheses with overlapped regions.) }
\end{itemize}


If $\hstar \in M_2$, we assume that the two rectangles of $\hstar$ never share an edge, so that the labels of the 12 corner points are consistent between the two rectangles.

\begin{itemize}
\item Teaching from $M_1$ to $M_1$:
  \begin{itemize}
  \item candidate examples are the 6 corners points.
  \item use negative examples only if all positive corners are consistent
  \item use the lower left positive corner only if
    \begin{itemize}
    \item the upper right positive corner is consistent or
    \item learner has to move the lower/left edges before moving the upper/right edges
    \end{itemize}
  \end{itemize}

\item Teaching from $M_2$ to $M_1$:
  \begin{itemize}
  \item if either of the two rectangles of $h_t$ is non-overlapping with the target $\hstar$:
    \begin{itemize}
    \item shrink -- pick the center point of any of the non-overlapping rectangles
    \end{itemize}
  \item otherwise, we know that both rectangles of $h_t$ are overlapping with $\hstar$:
    \begin{itemize}
    \item if either of the four corners of $\hstar$ is not fully aligned with $h_t$
      \begin{itemize}
      \item locate this rectangles $h$, set the intermediate target to be a half rectangle that only overlaps with $h$. Then, run the $M_1\rightarrow M_1$ algorithm, but only pick examples whose labeling is consistent between $h$ and $\hstar$.
      \end{itemize}
    \item if all four corners are fully aligned with $h_t$
      \begin{itemize}
      \item merge -- pick the center point of the vacancy region in the middle
      \end{itemize}
    \end{itemize}
  \end{itemize}
\item Teaching from $M_1$ to $M_2$:
  \begin{itemize}
  \item pick a rectangle in $\hstar$ that is not consistent with $h_t$, say $h$, use the $M_1 \rightarrow M_1$ teacher to find an example
  \end{itemize}
\end{itemize}


\begin{figure*}[!ht]
  \centering
  \includegraphics[height=2.5cm]{./fig/empty_boxes.pdf}
  \caption{Illustration of the preferred transitions according to our model of the learner $M(\sigma, \Hypotheses)$}
  \label{fig:rectangle_transition}
\end{figure*}
..\\
..\\
..\\




% \section{Global preference setting}
% Assume that there is a global preference of hypotheses (as a partial ordering of hypothesis in terms of preference). We use the following teaching protocol:

% Before the teaching starts, learner chooses a hypothesis from the top of the priority queue.

% At round $t$,
% \begin{itemize}\denselist
% \item (optional) Teacher observes the learner's current hypothesis $h_t$
% \item Teacher picks a teaching example
% \item The learner prunes away inconsistent hypotheses from the version space
% \item If needed, the learner chooses a hypothesis from the top of the priority queue.
% \end{itemize}
% The teaching process ends whenever the learner reaches $h^*$.

% Both non-adaptive and adaptive teaching strategy have the same complexity as PBTD.

% Argument: for the adaptive setting, the (local) adaptation is reset every iteration once the learner makes a jump according to the global preference ordering.


% \section{Local preference setting}

% Fix a starting state and target, we want to come up with an example where there is a difference between adaptive and non-adaptive.


% \begin{itemize}
% \item Teaching dimension (TD), preference based teaching dimension (PBTD): $\hypothesis^{t+1} \sim (\hypotheses^{t+1})$
% \item Local preference-based (LPB): $\hypothesis^{t+1} \sim (\hypotheses^{t+1}, \hypothesis^t)$
% \item LPB-Action: $\hypothesis^{t+1} \sim (\hypotheses^{t+1}, \hypothesis^t, x^t )$
% \end{itemize}


% \paragraph{Taxonomy} Try to come with an illustrative (real-world) example where adaptivity helps.
% \paragraph{$d$-dimensional grid world}
% Adaptive takes $\bigO(n)$, non-adaptive takes $\bigO(n^d)$
% \paragraph{Tree with an exponential number of target states}


% \section{Non-adaptive teacher}
% Non-adaptive teacher
% \begin{align}
%   \label{eq:1}
%   x^t = \argmin_{x\in \examples} \max_{h^t\in \hypotheses^t} \max_{h\in f(\hypotheses^t, h^t, x)} \text{rank}(\hypothesis^* \given \hypothesis, \hypotheses^t, \hypothesis^t, x^t)
% \end{align}

% % \begin{theorem}
% %   Lower bound for polynomial time non-adaptive algorithm.
% % \end{theorem}
% (optional) A non-adaptive teaching algorithm.

% If we include this, we need to discuss the stopping criterion for the non-adaptive teacher
% \begin{itemize}\denselist
% \item communicative teacher when $h^*$ is reached
% \item
% \end{itemize}


% \clearpage
% \subsection{Examples}
% \paragraph{Monomials with edit distance}
% \paragraph{Halfspaces}


% \section{The Adaptive Teaching Model}
% \subsection{Teaching Protocol}

% \begin{itemize}\denselist
% \item Learner starts with a hypothesis space $h_0\in \hypotheses$
% \item At time step $t$
%   \begin{itemize}
%   \item Teacher picks example $x_t$
%   \item Learner updates its hypothesis according to $M(\cdot)$: $h_t \rightarrow_M h_{t+1}$.
%   \item Teacher observes learner's hypothesis $h_{t+1}$
%   \end{itemize}
% \end{itemize}

% \subsection{Objective}
% \begin{align*}
%   \argmin_{|S|} S, \text{~s. t.~} \hypotheses(S) = \{\hypothesis^*\}
% \end{align*}

% \section{Main Result}
% \subsection{The Omniscient Teaching Dimension}
% \begin{definition}[Omniscient teaching dimension]
% \end{definition}

% \begin{theorem}
%   Suppose that learners moves according to the mobility constraint \text{mobi-constr}. The omniscient teaching dimension for version space learners is
%   $\bigO{\text{mobi-constr}\cdot \log{\frac{1}{\epsilon}}}$.
% \end{theorem}

% \subsection{Algorithm}





% Fix $\randomstate$. Denote the full teaching sequence of the optimal algorithm under preference $\ordering$ as $\examples^m = \{\example^1, \example^2, \dots, \example^m\}$, and the trace of the learner's hypotheses are $\{\hypothesis^1, \hypothesis^2, \dots, \hypothesis^m\}$.

% \underline{Case 1.} Assume that $\forall i \in \{1, \dots, {m-1}\}, \hinit(\instance_{\example^i}) = \lbl_{\example^i}$. That is, the optimal algorithm under preference $\ordering$ eliminates $\hinit$ at the last step, right before the learner reaches $\hstar$. Then, prior to eliminating $\hinit$, any teaching examples shown to the learner does not change the preference ordering over the consistent hypotheses in the preferred set $\prefset(\ordering, \hstar, \hinit, \Hypotheses)$. Applying the same set of teaching examples $\{\example^1, \example^2, \dots, \example^{m-1}\}$ in any order, followed by $\example^m$, is guaranteed to eliminate $\prefset(\ordering, \hstar, \hinit, \Hypotheses) \setminus \{\hstar\}$. By definition, $\optcost(\uordering, \hstar, \hinit, \prefset(\ordering, \hstar, \hinit, \Hypotheses))$ is the lower bound on the number of examples required to eliminate $\prefset(\ordering, \hstar, \hinit, \Hypotheses) \setminus \{\hstar\}$. It follows that $\optcost(\uordering, \hstar, \hinit, \prefset(\ordering, \hstar, \hinit, \Hypotheses)) \leq m$.

% \underline{Case 2.} Assume that $\example^t$ is the first example in $\examples^m$ that is inconsistent with $\hinit$, and $t < m$. According to Condition~\ref{thm:suffcond:1} of \thmref{thm:greedy_suff}, we know that any algorithm that eliminates $\hypothesis$ ends up with a larger preferred version space, compared with the




****************************

In the following, we will focus on the analysis of the greedy algorithm with preference $\ordering$.

% \begin{lemma}
%   %   $\futurecostapprox(\hypothesis^t, \Hypotheses(\examples^t \cup \{\example^t\}) \leq |\prefset(\uordering, \hypothesis^0, \hstar, \Hypotheses(\examples^t \cup \{\example^t\})|$
%   Assume that the preference function $\ordering$ and the structure of tests satisfy Condition 1 and 2 from \thmref{thm:greedy_suff}. Suppose we have run the greedy teacher for $m$ time steps. Let $\examples^m$ be the set of examples chosen by the greedy teacher, and $\hypothesis^m$ be the learner's current hypothesis. Then $\forall \example, |\prefset(\ordering, \hstar, \hypothesis^m,  \Hypotheses(\examples^m \cup \{\example\})| \leq |\prefset(\uordering, \hstar, \hypothesis^0,  \Hypotheses(\examples^m \cup \{\example\})|$.
% \end{lemma}
% \begin{proof}
We first show that at any two consecutive time steps $t-1, t$, it holds that $|\prefset(\ordering, \hstar, \hypothesis^{t-1}, \Hypotheses(\examples^t \cup \{\example\})| = |\prefset(\ordering, \hstar, \hypothesis^t,  \Hypotheses(\examples^t \cup \{\example\})|$.


\underline{Case 1: $\hypothesis^{t-1} = \hypothesis^{t}$.} The above result follows immediately.

\underline{Case 2: $\hypothesis^{t-1} \neq \hypothesis^{t}$.}
Since the teacher is following the greedy heuristic, we know
\begin{align*}
  |\prefset(\ordering, \hstar, \hypothesis^t,  \Hypotheses(\examples^{t}))| = \min_\example |\prefset(\ordering, \hstar, \hypothesis^{t-1},  \Hypotheses(\examples^{t-1}\cup\{\example\}))|
\end{align*}

We also know that example $\example^t$ is inconsistent with $\hypothesis^{t-1}$. According to Condition \ref{thm:suffcond:2} of \thmref{thm:greedy_suff}, there exists an example $\example'$, s.t., $\Hypotheses(\{\example'\})\setminus \Hypotheses(\{\example^t\}) = \{\hypothesis^{t-1}\}$. Combined with the above equation,
\begin{align}
  |\prefset(\ordering, \hstar, \hypothesis^t,  \Hypotheses(\examples^{t}))|
  &= \min_\example |\prefset(\ordering, \hstar, \hypothesis^{t-1},  \Hypotheses(\examples^{t-1}\cup\{\example\}))| \notag \\
  &\leq |\prefset(\ordering, \hstar, \hypothesis^{t-1},  \Hypotheses(\examples^{t-1}\cup\{\example'\}))| \notag \\
  &= |\prefset(\ordering, \hstar, \hypothesis^{t-1},  \Hypotheses(\examples^{t-1}\cup\{\example^t\}))| + 1 \notag \\
  &= |\prefset(\ordering, \hstar, \hypothesis^{t-1},  \Hypotheses(\examples^{t}))| + 1 \label{eq:greedy_jump}
\end{align}

By Condition~\ref{thm:suffcond:1} of \thmref{thm:greedy_suff} (and step (b) of Eq.~\eqref{eq:prefset:ht}), we get
% \begin{align*}
%   $\prefset(\ordering, \hstar, \hypothesis^{t-1}, \Hypotheses(\examples^t \cup \{\example\}) \subseteq \prefset(\ordering, \hstar, \hypothesis^t,  \Hypotheses(\examples^t \cup \{\example\}).$
% % \end{align*}
% Therefore,
% \begin{align}
%   |\prefset(\ordering, \hstar, \hypothesis^{t-1}, \Hypotheses(\examples^t \cup \{\example\}))| \leq |\prefset(\ordering, \hstar, \hypothesis^t,  \Hypotheses(\examples^t \cup \{\example\}))|\
% \end{align}
\begin{align*}
  \prefset(\ordering, \hstar, \hypothesis^{t-1}, \Hypotheses(\examples^t)) \subseteq \prefset(\ordering, \hstar, \hypothesis^t,  \Hypotheses(\examples^t)). % \label{eq:greedy_jump_extend}
\end{align*}
which leads to
\begin{align}
  |\prefset(\ordering, \hstar, \hypothesis^{t-1}, \Hypotheses(\examples^t))| \leq |\prefset(\ordering, \hstar, \hypothesis^t,  \Hypotheses(\examples^t))| \leq |\prefset(\ordering, \hstar, \hypothesis^{t-1}, \Hypotheses(\examples^t))| + 1. \label{eq:greedy_jump_extend}
\end{align}

Eq.~\eqref{eq:greedy_jump} and \eqref{eq:greedy_jump_extend} imply that, after the learner jumps to a new hypothesis (by receiving $\example^t$), the preferred version space can be extended by at most 1 hypothesis, compared to the preferred version space at the previous time step.

Further notice that in Eq.~\eqref{eq:greedy_jump_extend}, exactly one equality can hold. If $|\prefset(\ordering, \hstar, \hypothesis^{t-1}, \Hypotheses(\examples^t))| = |\prefset(\ordering, \hstar, \hypothesis^t,  \Hypotheses(\examples^t))|$, then $\prefset(\ordering, \hstar, \hypothesis^{t-1}, \Hypotheses(\examples^t)) = \prefset(\ordering, \hstar, \hypothesis^t,  \Hypotheses(\examples^t))$.

If $|\prefset(\ordering, \hstar, \hypothesis^{t-1}, \Hypotheses(\examples^t))| + 1 = |\prefset(\ordering, \hstar, \hypothesis^t,  \Hypotheses(\examples^t))|$



% Let us now consider a surrogate objective function, .


*************************************************

At each time step, greedy either
\begin{itemize}\denselist
\item remove a set of examples according to the greedy heuristic, add none
\item remove a set of examples, then add one
\end{itemize}


% $\prefset(\ordering, \hstar, \hypothesis^t,  \Hypotheses(\examples^t)) \leq \prefset(\ordering, \hstar, \hypothesis^{t-1},  \Hypotheses(\examples^{t}))$, i.e., moving to a different hypothesis $\hypothesis^t$ does not brings the learner further from $\hstar$, compared with

    %     the teaching example $\example^t$, because the teacher is .
% \end{proof}






% \begin{proof}
We first show that at any two consecutive time steps $t-1, t$, it holds that $|\prefset(\ordering, \hstar, \hypothesis^{t-1}, \Hypotheses(\examples^t \cup \{\example\})| = |\prefset(\ordering, \hstar, \hypothesis^t,  \Hypotheses(\examples^t \cup \{\example\})|$.


\underline{Case 1: $\hypothesis^{t-1} = \hypothesis^{t}$.} The above result follows immediately.

\underline{Case 2: $\hypothesis^{t-1} \neq \hypothesis^{t}$.}
% Since the teacher is following the greedy heuristic, we know
% \begin{align*}
    %     |\prefset(\ordering, \hstar, \hypothesis^t,  \Hypotheses(\examples^{t}))| = \min_\example |\prefset(\ordering, \hstar, \hypothesis^{t-1},  \Hypotheses(\examples^{t-1}\cup\{\example\}))|
    %   \end{align*}

We know that example $\example^t$ is inconsistent with $\hypothesis^{t-1}$. According to Condition \ref{thm:suffcond:2} of \thmref{thm:greedy_suff}, there exists an example $\example'$ which is consistent with $\hypothesis^{t-1}$, and $\Hypotheses(\{\example'\})\setminus \Hypotheses(\{\example^t\}) = \{\hypothesis^{t-1}\}$. Since the teacher is following the greedy heuristic, we know that
\begin{align}
  |\prefset(\ordering, \hstar, \hypothesis^t,  \Hypotheses(\examples^{t-1}\cup \{\example^t\}))|
  &\leq |\prefset(\ordering, \hstar, \hypothesis^{t-1},  \Hypotheses(\examples^{t-1}\cup\{\example'\}))| \notag \\
  &= |\prefset(\ordering, \hstar, \hypothesis^{t-1},  \Hypotheses(\examples^{t-1}\cup\{\example^t\}))| + 1 \notag \\
  &= |\prefset(\ordering, \hstar, \hypothesis^{t-1},  \Hypotheses(\examples^{t}))| + 1 \label{eq:greedy_jump}
\end{align}


Combined with the above equation,
\begin{align}
  |\prefset(\ordering, \hstar, \hypothesis^t,  \Hypotheses(\examples^{t}))|
  &= \min_\example |\prefset(\ordering, \hstar, \hypothesis^{t-1},  \Hypotheses(\examples^{t-1}\cup\{\example\}))| \notag \\
  &\leq |\prefset(\ordering, \hstar, \hypothesis^{t-1},  \Hypotheses(\examples^{t-1}\cup\{\example'\}))| \notag \\
  &= |\prefset(\ordering, \hstar, \hypothesis^{t-1},  \Hypotheses(\examples^{t-1}\cup\{\example^t\}))| + 1 \notag \\
  &= |\prefset(\ordering, \hstar, \hypothesis^{t-1},  \Hypotheses(\examples^{t}))| + 1 \label{eq:greedy_jump}
\end{align}

By Condition~\ref{thm:suffcond:1} of \thmref{thm:greedy_suff} (and step (b) of Eq.~\eqref{eq:prefset:ht}), we get
    %     \begin{align*}
    %     $\prefset(\ordering, \hstar, \hypothesis^{t-1}, \Hypotheses(\examples^t \cup \{\example\}) \subseteq \prefset(\ordering, \hstar, \hypothesis^t,  \Hypotheses(\examples^t \cup \{\example\}).$
    % %   \end{align*}
    %     Therefore,
    %     \begin{align}
    %     |\prefset(\ordering, \hstar, \hypothesis^{t-1}, \Hypotheses(\examples^t \cup \{\example\}))| \leq |\prefset(\ordering, \hstar, \hypothesis^t,  \Hypotheses(\examples^t \cup \{\example\}))|\
    %   \end{align}
\begin{align*}
  \prefset(\ordering, \hstar, \hypothesis^{t-1}, \Hypotheses(\examples^t)) \subseteq \prefset(\ordering, \hstar, \hypothesis^t,  \Hypotheses(\examples^t)). % \label{eq:greedy_jump_extend}
\end{align*}
which leads to
\begin{align}
  |\prefset(\ordering, \hstar, \hypothesis^{t-1}, \Hypotheses(\examples^t))| \leq |\prefset(\ordering, \hstar, \hypothesis^t,  \Hypotheses(\examples^t))| \leq |\prefset(\ordering, \hstar, \hypothesis^{t-1}, \Hypotheses(\examples^t))| + 1. \label{eq:greedy_jump_extend}
\end{align}

Eq.~\eqref{eq:greedy_jump} and \eqref{eq:greedy_jump_extend} imply that, after the learner jumps to a new hypothesis (by receiving $\example^t$), the preferred version space can be extended by at most 1 hypothesis, compared to the preferred version space at the previous time step.

Further notice that in Eq.~\eqref{eq:greedy_jump_extend}, exactly one equality can hold. If $|\prefset(\ordering, \hstar, \hypothesis^{t-1}, \Hypotheses(\examples^t))| = |\prefset(\ordering, \hstar, \hypothesis^t,  \Hypotheses(\examples^t))|$, then $\prefset(\ordering, \hstar, \hypothesis^{t-1}, \Hypotheses(\examples^t)) = \prefset(\ordering, \hstar, \hypothesis^t,  \Hypotheses(\examples^t))$.

If $|\prefset(\ordering, \hstar, \hypothesis^{t-1}, \Hypotheses(\examples^t))| + 1 = |\prefset(\ordering, \hstar, \hypothesis^t,  \Hypotheses(\examples^t))|$



    %     Let us now consider a surrogate objective function, .





%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:

